MaViLS, a Benchmark Dataset for Video-to-Slide Alignment, Assessing Baseline Accuracy with a Multimodal Alignment Algorithm Leveraging Speech, OCR, and Visual Features

This paper presents a benchmark dataset for aligning lecture videos with corresponding slides and introduces a novel multimodal algorithm leveraging features from speech, text, and images. It achieves an average accuracy of 0.82 in comparison to SIFT (0.56) while being approximately 11 times faster. Using dynamic programming the algorithm tries to determine the optimal slide sequence. The results show that penalizing slide transitions increases accuracy. Features obtained via optical character recognition (OCR) contribute the most to a high matching accuracy, followed by image features. The findings highlight that audio transcripts alone provide valuable information for alignment and are beneficial if OCR data is lacking. Variations in matching accuracy across different lectures highlight the challenges associated with video quality and lecture style. The novel multimodal algorithm demonstrates robustness to some of these challenges, underscoring the potential of the approach.

==> rebuttal.tex <==
Rebuttal

Thanks to all reviewers for their insightful feedback. Regarding concerns from one reviewer about the size of our dataset compared to the one cited in https://arxiv.org/abs/2208.08080, we recognize the benefits of larger datasets but want to highlight the unique strength of our own dataset. Our dataset encompasses contributions from 20 different lecturers all from different academic domains and contains 850 slides in total. In contrast, the dataset referenced by the reviewer includes data from only 10 lecturers within only 6 domains. For testing robustness of video-to-slide alignment, our goal was to create a rich dataset, rather than having more slides from the same lecturer or domain. Additionally, our dataset is diverse with respect to image-to-text ratio, sound and image quality, volatility score that measures jumping back and forth within slides and the ratio between slide to non-slide view. 

The dataset, as well as the code will be published on GitHub as soon as the blind-review process is over in order to ensure transparency and facilitate further research in this area.






